Dendron: Enhancing Human Activity Recognition with On-Device TinyML Learning

Human activity recognition (HAR) is a research field that employs Machine Learning (ML) techniques to identify user activities. Recent studies have prioritized the development of HAR solutions directly executed on wearable devices, enabling the on-device activity recognition. This approach is supported by the Tiny Machine Learning (TinyML) paradigm, which integrates ML within embedded devices with limited resources. However, existing approaches in the field lack in the capability for on-device learning of new HAR tasks, particularly when supervised data are scarce. To address this limitation, our paper introduces Dendron, a novel TinyML methodology designed to facilitate the on-device learning of new tasks for HAR, even in conditions of limited supervised data. Experimental results on two public-available datasets and an off-the-shelf device (STM32-NUCLEO-F401RE) show the effectiveness and efficiency of the proposed solution.

==> external_files/on-device_comparison_2.tex <==
\begin{table}[h]
    \centering
    \caption{Minutes per task for the on-device learning evaluation presented in Section \ref{sec:on-device_learning_ev}}    \label{tab:minute_per_task}
    \begin{tabular}{|ccc|}
        \hline
        Dataset & downstairs vs upstairs & sit-to-stand vs stand-to-sit\\
        \hline\hline
        \textbf{UCA-EHAR} & $40$ min & $4$ min\\
        
        \textbf{UCI-HAPT} & $48$ min\footnotemark & $24$ min\\
        \hline
    \end{tabular}
    
\end{table}

\footnotetext{The UCI-HAPT dataset has $\approx 480$ minutes for walking upstairs vs. downstairs, but only 10\% was used for the evaluation in Section \ref{sec:on-device_learning_ev} to simulate supervised data scarcity condition.}

==> external_files/table_comparison_hier.tex <==
\begin{table}[t]
    \caption{Performance comparison between the hierarchical solution and \textit{Dendron}.
    (\textit{Figure \ref{fig:hier-example-fig} contains tasks specifications})}
    \label{table:comparison_hier}
   \centering 

    \begin{tabular}{|cc|c| c c c c c c |}
    \hline
    % \multicolumn{4}{|c|}{\textbf{\networkNameNoSpace}}\\
     \multicolumn{3}{|c|}{} & $T^{(1)}$& $T^{(2)}$ &$T^{(3)}$& $T^{(4)}$&$T^{(5)}$&$T^{(6)}$\\
     \hline\hline
     \multicolumn{3}{|c|}{num. samples/task}&$42$k&$21$k&$22$k&$16$k&$16$k&$5$k\\
     \hline\hline
     \multicolumn{2}{|c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\shortstack[l]{\scriptsize Hierarchical\\Solution}}}}
    % \multirow{4}{*}{\rotatebox[origin=c]{90}{\shortstack[l]{Hierarchical\\Solution}}}
    &accuracy&$0.99$&$0.99$&$0.95$&$0.63$&$0.68$&$0.90$\\
    &&precision&$0.99$&$0.99$&$0.92$&$0.66$&$0.82$&$0.83$\\
    &&recall&$0.99$&$0.99$&$0.84$&$0.94$&$0.68$&$0.99$\\
    &&F1-score&$0.99$&$0.99$&$0.88$&$0.78$&$0.74$&$0.90$\\
    \hline
    \hline
    \multicolumn{2}{|c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\shortstack[l]{\scriptsize \textbf{Dendron}}}}}
    &accuracy&$0.99$&$0.96$&$0.95$&$0.63$&$0.86$&$0.89$\\
    &&precision&$0.98$&$0.57$&$0.84$&$0.52$&$0.80$&$0.87$\\
    &&recall&$0.99$&$0.73$&$0.79$&$0.35$&$0.89$&$0.97$\\
    &&F1-score&$0.98$&$0.64$&$0.82$&$0.42$&$0.84$&$0.92$\\
   
    \hline
    % \multicolumn{6}{c}{}\\
    % \multicolumn{6}{c}{}\\
    \end{tabular}
    
    
    
\end{table}

==> external_files/table_comparison_hier_2.tex <==

% \begin{table*} [t]
%     \caption{Performance comparison between the single-model solution, the hierarchical solution, and \textit{Dendron}.}
%     \label{table:comparison_hier}
%    \centering 

%   \begin{tabular}{|c|S[table-format=6]|c|c|c|c|}
%         \hline
%         \multirow{2}{*}{Class} &  \multicolumn{2}{c|}{Num. samples} & \multicolumn{3}{c|}{Class accuracy} \\
%         \cline{2-6}
%         &Training&Testing&Single-model&Hierarchical&\textbf{Dendron}\\
%         \hline\hline
%         Sitting&21680&6949&$0.50$&$\bm{0.78}$&$0.40$\\
%         Standing&12496&3699&$0.60$&$0.21$&$\bm{0.63}$\\
        
%         \hline\hline
        
%         Lying&10661&3021&$0.92$&$0.95$&$\bm{1.00}$\\
        
%         Running&11917&3423&$\bm{0.97}$&$0.90$&$0.92$\\
        
%         Walking&24848&7337&$0.91$&$\bm{0.94}$&$\bm{0.94}$\\
        
%         Walking downstairs&5111&1421&$\bm{0.87}$&$0.80$&$0.76$\\
        
%         Walking upstairs&5685&1737&$0.68$&$0.61$&$\bm{0.78}$\\
%        \hline
%   \end{tabular}
    
    
    
% \end{table*}


\begin{table}
    \caption{Off-Device classification performances comparison between the single-model solution, the hierarchical solution, and Dendron.}
    \label{table:off_device_evaluation}
    \centering
    \begin{tabular}{|ccccc|}
         \hline
         \multicolumn{2}{|c}{}&Single-model & Hierarchical & \textbf{Dendron}\\
         \hline\hline
         \multirow{7}{*}{\textbf{UCA}}&Sitting& $0.73 \pm 0.015$& -& -\\
         &Standing& $0.74 \pm 0.004$& -&-\\
         &Laying& $0.74 \pm 0.004$& -& -\\
         &Running& $0.74 \pm 0.004$& -& -\\
         &Walking& $0.74 \pm 0.004$& -& -\\
         &Up& $0.74 \pm 0.004$& -& -\\
         &Down& $0.74 \pm 0.004$& -& -\\

        
         \hline\hline
         \multirow{7}{*}{\textbf{UCI}}&Accuracy& -& -& -\\
         &standing& $0.74 \pm 0.004$& -& -\\
         &standing& $0.74 \pm 0.004$& -& -\\
         &standing& $0.74 \pm 0.004$& -& -\\
         &standing& $0.74 \pm 0.004$& -& -\\
         &standing& $0.74 \pm 0.004$& -& -\\
         &standing& $0.74 \pm 0.004$& -& -\\
         \hline
    \end{tabular}
\end{table}

==> external_files/table_comparisons.tex <==
\begin{table}[t]
    \caption[prova]{Comparison in terms of memory, computation, and latency using the STM32-NUCLEO-F401RE\\
    \textit{$M_{\text{FE}}^{(i)}$, $C_{\text{FE}}^{(i)}$, $M_{\text{FC}}^{(i)}$, and $C_{\text{FC}}^{(i)}$ are respectively the memory, and computation load of the $i-th$ task for the feature extractor (FE), and the fully connected (FC) modules.\footnotemark}}
    \label{table:comparison}
   \centering 

    \begin{tabular}{|c| c| c |c |}
    \hline
    % \multicolumn{4}{|c|}{\textbf{\networkNameNoSpace}}\\
     & Memory& \multirow{2}{*}{\shortstack[l]{Computation\\(MACC)}} & \multirow{2}{*}{\shortstack[l]{Mean\\Latency}}\\
     &&&\\
    \hline\hline
     \multirow{2}{*}{\shortstack[l]{Single-model\\solution}} & $M_{\text{FE}} + M_{\text{FC}}$ &$C_{\text{FE}} + C_{\text{FC}}$ & \multirow{2}{*}{$\approx47$ ms}\\
     &$\approx60$ KiB&$\approx427,242$&\\
     \hline
     \multirow{2}{*}{\shortstack[l]{Hierarchical\\solution}} & $\sum_{i}^{n} M_{\text{FE}}^{(i)} + M_{\text{FC}}^{(i)}$ &$\sum_{i} C_{\text{FE}}^{(i)} +  C_{\text{FC}}^{(i)}$ & \multirow{2}{*}{$\approx94$ ms}\\
    &$\approx 324$ KiB&$\approx851,292$&\\
    
    \hline
   
    \hline
     \multirow{2}{*}{\textbf{Dendron}} & $\pmb{M_{\text{FE}} + \sum_{i}^{n} M_{\text{FC}}^{(i)}}$ &$\pmb{C_{\text{FE}} + \sum_{i} C_{\text{FC}}^{(i)}}$ & \multirow{2}{*}{$\pmb{\approx47 \text{ ms}}$}\\
    &$\pmb{\approx67\text{ KiB}}$&$\pmb{\approx426,444}$&\\

    \hline
    % \multicolumn{6}{c}{}\\
    % \multicolumn{6}{c}{}\\
    \end{tabular}    
    
\end{table}

\footnotetext{The notation $\sum_{i}$ denotes a summation over a specific subset of task indexes, while $\sum_{i}^{n}$ represents the summation over all task indexes.}
